Efficient Multi-Agent Collaboration with Tool Use for Online Planning in Complex Table Question Answering

Complex table question answering (TQA) aims to answer questions that require complex reasoning, such as multi-step or multi-category reasoning, over data represented in tabular form. Previous approaches demonstrated notable performance by leveraging either closed-source large language models (LLMs) or fine-tuned open-weight LLMs. However, fine-tuning LLMs requires high-quality training data, which is costly to obtain, and utilizing closed-source LLMs poses accessibility challenges and leads to reproducibility issues. In this paper, we propose Multi-Agent Collaboration with Tool use (MACT), a framework that requires neither closed-source models nor fine-tuning. In MACT, a planning agent and a coding agent that also make use of tools collaborate to answer questions. Our experiments on four TQA benchmarks show that MACT outperforms previous SoTA systems on three out of four benchmarks and that it performs comparably to the larger and more expensive closed-source model GPT-4 on two benchmarks, even when using only open-weight models without any fine-tuning. We conduct extensive analyses to prove the effectiveness of MACT's multi-agent collaboration in TQA.

==> tex/6-analysis.tex <==
\section{Analysis}
To understand our framework better, i.e., which components contribute to the performance to which extent, we conduct different analyses.
Unless mentioned explicitly, all experiments are done on Qwen 70b with codellama 34b \heiketodo{with Qwen 70b as the planning and codellama 34b as the coding agent}, with sampling size $k=5$, selection model $f_s = \text{self consistency}$, and the efficiency parameter $\alpha>1$ (which means we use our framework on all instances).
\subsection{Agent collaboration}
One very difference between our approach and previous work is that we propose a multi-agent setting.
To test the effectiveness of multi-agent as well as adding tools, we provide an ablation study: 1) Ablating the searching and calculating tools and replacing them with the planing agent. 
2) Removing the coding agent further and replacing it with the planning agent. 
The results are shown in Table \ref{tab:ablation}.

We find that the multi-agent set up with tool usages can indeed enhance the performance.
This is proved by the dropping results when ablating them. 
Interestingly, the effect of adding the coding agent and external tools varies across different data sets and model sizes. 
For instance, there is a larger gap between when ablating the coding agent and tools for WTQ and TAT, than for CRT and SCITAB.  
This might be because of the data set features: CRT has lots of yes-no questions and SCITAB is a trinary classification data set.
As a result, it is more likely for model to 'guess' the final answer in these two data sets than WTQ and TAT.
To prove that, we calculate the accuracy of the models on instances that having answers other than yes and no from CRT when ablating both the coding agent and tools.
This results in a drop of 6.43 (39.59 with tool v.s. 33.16 without tool) for the small model, and a drop of 7.7 (52.19 with tool v.s. 44.47 without tool) for the larger model. \heiketodo{v.s. $\rightarrow$ vs.\ (the backslash avoids that Latex creates a longer whitespace after the dot)}

We also find that there is a smaller drop when ablating the coding agent and tools for the larger model than for the smaller model for most of the data sets.
This is not surprising as the larger models are more powerful in terms of arithmetic, commonsense reasoning, as well as retrieving information from tables. 
The observations indicates our framework helps small models more than the larger models. 



\begin{table}[!t]
\heiketodo{use w/o instead of -}
\centering
\small
  \begin{tabular}{lcccc}
    \toprule
      & \textbf{WTQ} &  \textbf{TAT} &  \textbf{CRT}&  \textbf{SCITAB}\\
    \midrule
    % planning agent, coding agent, tool use, collobaration
    Ours (small)& 61.74 & 61.58 & 52.34 &53.27 \\ \cmidrule{2-5}
    \hspace{2mm} -Tool & \makecell{58.31\\(\textcolor{red}{-3.43})} &\makecell{ 53.10\\(\textcolor{red}{-8.48})}&\makecell{52.47\\(\textcolor{red}{+0.13})} & \makecell{52.12\\(\textcolor{red}{-0.15})}\\  \cmidrule{2-5}
    \hspace{2mm} - Code - Tools & \makecell{52.87\\(\textcolor{red}{-8.88})} & \makecell{49.91\\(\textcolor{red}{-11.67})}&\makecell{50.96\\(\textcolor{red}{-1.65})} &\makecell{50.25\\(\textcolor{red}{-3.02})}\\
    %\textsc{sep-sc}$\lozenge$ & & 51.41& 50.27& \\
    %\textsc{sep-tex}$\lozenge$ &  &48.83& 50.41&\\
    \midrule
    Ours (large) & 72.63  & 66.21 & 64.42 & 59.80 \\\cmidrule{2-5}
     \hspace{2mm} - Tools & \makecell{71.32\\(\textcolor{red}{-1.31})}& \makecell{64.34\\(\textcolor{red}{-1.87})} & \makecell{63.87\\(\textcolor{red}{-0.55})}& \makecell{58.17\\(\textcolor{red}{-1.63})} \\  \cmidrule{2-5}
     \hspace{2mm} - Code - Tools  & \makecell{67.13\\(\textcolor{red}{-5.5})}& \makecell{61.15\\(\textcolor{red}{-5.06})} & \makecell{60.44\\(\textcolor{red}{-3.98})} &\makecell{57.92\\(\textcolor{red}{-1.88})}\\
    %\textsc{sep-sc} & &53.28 & 60.99& \\
    %\textsc{sep-tex} &  &53.16 & 55.77&\\
    %    \textsc{sep-code} &  &29.52 &49.59 &\\
    \bottomrule
  \end{tabular}
\caption{Collaboration effect: results of different settings. settings with $\lozenge$ use a smaller plan agent: Qwen 7b. Otherwise, Qwen 72b is used as the plan agent.}
\label{tab:ablation}
\end{table}


% \begin{table}[!t]
% \centering
% \small
%   \begin{tabular}{lcccc}
%     \toprule
%       & \textbf{WTQ} &  \textbf{TAT} &  \textbf{CRT}&  \textbf{SCITAB}\\
%     \midrule
%     original (7b)& 61.74 & 61.58 & 52.34 &53.27 \\
%     - code and tools (7b) & 52.87 & 49.91&50.96 &50.25\\
%     %\textsc{sep-sc}$\lozenge$ & & 51.41& 50.27& \\
%     %\textsc{sep-tex}$\lozenge$ &  &48.83& 50.41&\\
%     \midrule
%     original (70b) & 72.63  & 66.21 & 64.42 & 59.80 \\
%     -code and tools (70b) & 67.13& 61.15 & 60.44 &57.92\\
%     %\textsc{sep-sc} & &53.28 & 60.99& \\
%     %\textsc{sep-tex} &  &53.16 & 55.77&\\
%     %    \textsc{sep-code} &  &29.52 &49.59 &\\
%     \bottomrule
%   \end{tabular}
% \caption{Collaboration effect: results of different settings. settings with $\lozenge$ use a smaller plan agent: Qwen 7b. Otherwise, Qwen 72b is used as the plan agent.}
% \label{tab:result_collaboration}
% \end{table}


\subsection{Selection model}
\label{selection_model}
We experiment with different selection models. 
The results are shown in Table \ref{tab:result_selection}.

\begin{table}[!t]
\centering
%\resizebox{\columnwidth}{!}{%
  \begin{tabular}{@{}lcccc@{}}
    \toprule
      & \textbf{WTQ} &  \textbf{TAT} &  \textbf{CRT}&  \textbf{SCITAB}\\
    \midrule
    \textsc{sc}& 72.63 & 66.21 & 64.42 &59.80 \\
    \textsc{llm} & & & &\\
    \textsc{log\_p} & & & & \\
    \textsc{roll\_out} & & & & \\
    \textsc{combined} &  & & &\\
    \bottomrule
  \end{tabular}
%}
\caption{
}
\label{tab:result_selection}
\end{table}


\subsection{Sampling size}
We experiment with different sampling sizes.

\subsection{Efficiency parameter}

Though sampling and step-wise planning are promising in performance improvement \citep{Liu2023RethinkingTD,wu2024protrix}, it can become inefficient if the question is simple and can be easily addressed by the planning agent without the assistance of the coding agent and tools. 
To find a balance between accuracy and efficiency, we introduce a parameter $\alpha$ for invoking the planning loop. 
The intuition is that we do not need to invoke the planning loop when the model is confident. 
We measure model confidence by calculating the percentage of the most agreed answers. 
This is done by rolling out each planning trace at the first step until the final answer is obtained or the maximal step number is reached. 
\MMN{This is a very interesting and important feature of the approach if we have enough experiments about it.}





To understand how does the efficiency parameter $\alpha$ influence the performance, \heiketodo{to understand the impact of the efficiency parameter $\alpha$ on the performance} i.e., to find out the sweetspot \heiketodo{to investigate the trade-off} between efficiency and accuracy, we plot the model performance against $\alpha\in \{0.2, 0.4, 0.6, 0.8, 1\}$.
Remember that $\alpha$ stands for the percentage of the most agreed answer from the plan agent, the higher the $\alpha$, the more confident the plan agent, as the number of the most agreed answer is larger.\annetodo{instead plot number of votes used on x-axis}
The results are shown in Figure \ref{fig:efficiency}

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figs/tikz2.pdf}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

% wtq 70b
% 67.31  68.85  70.62  72.31  72.63  72.63
% 52.99  56.28  60.59  62.15  62.45  61.74
% crt 70b 
% 60.44  62.22, 63.46 64.56 65.25   64.42
% tat 70b 
% 61.15  62.30 63.38  65.30  66.51  66.21
% scitab 70b
%57.92 57.84 58.50 59.48 59.80 59.72

\subsection{Number of steps}
We report the distribution of numbers of steps for each dataset in Figure \ref{fig:iteration}.
As can be seen from the Figure, all instances can be solved within seven steps.
Data set wise, CRT and SCITAB feature bigger distribution of larger steps than WTQ and TAT, indicating their difficulties in terms of reasoning. 

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figs/step_dist.pdf}
    \caption{The distribution of number of steps for each data set.}
    \label{fig:iteration}
\end{figure}


%===================================
%Dataset
% wtq
% 1 0.211864406779661
% 2 58.3804143126177
% 3 36.95856873822976
% 4 3.5781544256120528
% 5 0.6826741996233522
% 6 0.14124293785310735
% 7 0.047080979284369114

%tat
% 1 0.30156815440289503
% 2 49.09529553679132
% 3 48.31121833534379
% 4 2.0506634499396865
% 5 0.24125452352231602

%crt
%2 18.549511854951188
% 3 45.467224546722456
% 4 23.570432357043238
% 5 9.06555090655509
% 6 2.789400278940028
% 7 0.5578800557880056

%scitab
% 1 3.4482758620689653
% 2 9.75609756097561
% 3 37.258200168208575
% 4 31.62321278385198
% 5 12.195121951219512
% 6 3.700588730025231
% 7 2.0185029436501263

%Feature??

\subsection{LLM as evaluator}
As mentioned before, using the exact match as evaluation metrics might not be optimal, as the correct answers can be expressed in various ways.
For instance, one question in the TAT data set asks \textit{What are the number of shares beneficially owned by L. Gordon Crovitz and Donald P. Hutchison respectively?}
The ground truth answer is \textit{16,016, 326,584} and our model predicts \textit{16,016 for Brian Kinion and 326,584 for Christopher Lien}. \heiketodo{why is it correct? shouldn't it include the entities from the question?}
Though the predicted answer is correct, it is deemed as incorrect using the exact match.
Therefore, we use GPT-4 as the evaluator to estimate the real performance of our model. 
The prompt we use can be found in the Appendix. 
The results are shown in Table \ref{tab:llm_evaluator}. 
We do not include SCITAB as the labels only feature three classes. \heiketodo{why not just include it to avoid having to motivate why you don't include it? ;)}
From the table, we find the performance on all of the three data sets increase.
There is a larger increase on TAT than the other data sets.
This is no surprise as the answers in this data set feature more flexible and longer expressions.



% EVALUATION = """ You are given a table, a question and optionally some texts about the table. 
% The gold answer to the question as well as a predicted answer are also provided. 
% Your task is to evaluate if the predicted answer is correct or not according to the gold answer.
% For numerical values, round the number to two demical places and if the difference between the two number is smaller than or equal to 0.01, then the prediction should be deemed as correct.
% Return simply correct or incorrect and do not carry out any reasoning to solve the question yourself.
% Table:{table}
% Text: {text}
% Question: {question}
% Gold answer: {gold_answer}
% Pred answer: {pred_answer}
% """

\begin{table}[!t]
\centering
%\resizebox{\columnwidth}{!}{%
  \begin{tabular}{@{}lccc@{}}
    \toprule
      & \textbf{WTQ} &  \textbf{TAT} &  \textbf{CRT}\\
    \midrule
    \textsc{sc}& 72.63 & 66.21 & 64.42 \\
    \textsc{llm} &77.83 & 87.85& 66.57\\
    \bottomrule
  \end{tabular}
%}
\caption{
}
\label{tab:llm_evaluator}
\end{table}

\subsection{Error analysis}

% crt 7b with tool
% 0.6814159292035398
% 0.39588688946015427

% crt 7b without tool
% 0.7138643067846607
% 0.33161953727506427


%crt 70b with tool
%0.7905604719764012
%0.5218508997429306

%crt 70b without tool
%0.799410029498525
%0.44473007712082263



==> tex/commands_old.tex <==
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\camerareadyblue}[1]{\textcolor{black}{#1}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\orange}[1]{\textcolor{black!20!orange}{#1}}

% Colored todonotes
\usepackage{todonotes}
\definecolor{talita}{rgb}{0.635,0.998,0.722}
\definecolor{anne}{rgb}{0.8,0.8,1}
\definecolor{sophie}{rgb}{0.998,0.722,0.635}
\definecolor{heike}{rgb}{0.4, 0.8, 0.4}
\definecolor{jakob}{rgb}{0.8,0.4,0.7}
\definecolor{steffen}{rgb}{0.2,0.4,0.8}
\definecolor{final}{rgb}{1, 1, 0.6}

\newcommand{\talitatodo}[2][talita]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}
\newcommand{\annetodo}[2][anne]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}
\newcommand{\sophietodo}[2][sophie]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}
\newcommand{\heiketodo}[2][heike]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}
\newcommand{\jakobtodo}[2][jakob]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}
\newcommand{\steffentodo}[2][steffen]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}
\newcommand{\finaltodo}[2][final]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}


==> tex/initial_explore.tex <==
\section{Initial investigation}
\textbf{Question: Is complex reasoning in TQA really a problem for LLMs? If so, what are the challenges?}

\paragraph{Method} We randomly sample 200 questions from the WTQ training and development set\footnote{training and seen table files} and extract corresponding single-step questions that only need operation to be solved in SQA. The motivation is that since SQA is constructed by decomposing multi-step questions in WTQ, comparing task performance on a set of questions only requiring single step operations with questions requiring multi-step complex reasoning, we can gain some insights about llm' capabilities in tacking questions with different levels of difficulties. We ensure that: 1) Each question in SQA only requires single-step operation without reasoning involved. This is achieved by manual annotation. 2) Each question in SQA corresponds to only one question in WTQ and vise versa and the SQA question is the decomposed version of the question in WTQ. 3) Each question in the sampled WTQ set is annotated with reasoning type (no reasoning/numerical/commonsense/temporal).  We conduct the initial experiment on the TableLlaMa for zero-shot. Neither WTQ nor SQA was used for training the model. We use exact match as the measurement for task performance.

\paragraph{Results and error analysis} For exact match, the results are \textbf{0.72} and \textbf{0.44} for SQA questions and WTQ questions respectively. This provides direct evidence that \textbf{complex reasoning is challenging for LLMs in TQA}. We further look into the percentage of questions the model in(correctly) predicted in each setting and what type of reasoning is involved. We find that among the questions the model predicted correctly in both settings (s1), 37 do not need reasoning, 30 require comparisons among values and 1 require commonsense reasoning. However, when looking at the questions where the model predicted incorrectly in the WTQ setting but correctly in the SQA setting (s2), the number of questions requiring reasoning increased: 65 of them require comparisons and 11 do not need any reasoning. This again proves that complex reasoning is challenging in TQA. Lastly, we categorize the errors LLMs made in s2. 
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
                    & SQA correct & SQA incorrect \\\hline
         WTQ correct&  0.38 (s1)    &  0.1 (s3)          \\
       WTQ incorrect&  0.34 (s2)      &  0.18 (s4)         \\
    \end{tabular}
    \caption{Percentage of questions for each setting.}
    \label{tab:my_label}
\end{table}

\begin{enumerate}
    \item comparing and arithmetic: though the model is capable of extract relevant information, it makes the majority of errors in comparing numerical or temporal information, as well as conducting arithmetic operations.   
    \item mapping between question and column header: the model fails to locate the correct header for information.
    \item extraction error: the model is not a perfect extractor, it can return the answer not grounded by the table; locate the neighboring cells of the relevant information and seems to have problems understanding temporal information. 
\end{enumerate}

% co_inco
% Counter({'compare': 65, 'extract': 11})
% co_co
% Counter({'extract': 37, 'compare': 30, 'commonsense': 1})
% inco_co
% Counter({'compare': 10, 'extract': 10})
% inco_inco
% Counter({'compare': 19, 'extract': 17})

==> tex/prior_work.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l|ccc}
    \toprule
     & \textbf{\datasetname} & \textbf{\blind} & \textbf{\cladder} \\
    \midrule
    \textit{Categorical distributions} & \green{\checkmark} & \red{\crossmark} & \red{\crossmark}\\
    \textit{Rung of causations} & \red{\crossmark} & \red{\crossmark} & \green{\checkmark} \\
    \textit{NL uncertainty} & \green{\checkmark} & \red{\crossmark} & \red{\crossmark}\\
    \textit{Symbolic target repr.} & \green{\checkmark} & \green{\checkmark} & \red{\crossmark} \\
    \textit{Topic/Domain variety} & \green{\checkmark} & \red{\crossmark} & \green{\checkmark} \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of \datasetname, \blind, and \cladder~ \red{Think if reasoning patterns are also category}}
    \label{tab:dataset_comparison}
\end{table}


\begin{itemize}
    \item Prior TQA systems (technical categories!)
    \item Datasets
\end{itemize}
